SCOOP: A Framework for Proactive Collaboration and Social Continual Learning through Natural Language Interaction andCausal Reasoning

Multimodal information-gathering settings, where users collaborate with AI in dynamic environments, are increasingly common. These involve complex processes with textual and multimodal interactions, often requiring additional structural information via cost-incurring requests. AI helpers lack access to users' true goals, beliefs, and preferences and struggle to integrate diverse information effectively. We propose a social continual learning framework for causal knowledge acquisition and collaborative decision-making. It focuses on autonomous agents learning through dialogues, question-asking, and interaction in open, partially observable environments. A key component is a natural language oracle that answers the agent's queries about environmental mechanisms and states, refining causal understanding while balancing exploration or learning, and exploitation or knowledge use. Evaluation tasks inspired by developmental psychology emphasize causal reasoning and question-asking skills. They complement benchmarks by assessing the agent's ability to identify knowledge gaps, generate meaningful queries, and incrementally update reasoning. The framework also evaluates how knowledge acquisition costs are amortized across tasks within the same environment. We propose two architectures: 1) a system combining Large Language Models (LLMs) with the ReAct framework and question-generation, and 2) an advanced system with a causal world model, symbolic, graph-based, or subsymbolic, for reasoning and decision-making. The latter builds a causal knowledge graph for efficient inference and adaptability under constraints. Challenges include integrating causal reasoning into ReAct and optimizing exploration and question-asking in error-prone scenarios. Beyond applications, this framework models developmental processes combining causal reasoning, question generation, and social learning.

==> pseudocode.tex <==

\begin{algorithm}[H]
\caption{Main ReAct Loop with \texttt{CausalRefinementAndAction}}
\label{alg:react-causal}
\begin{algorithmic}[1]
\STATE \textbf{Inputs:}
\STATE \quad User prompt $\mathcal{U}$, environment description $\mathcal{E}$, optional multimodal data
\STATE \quad Causal Knowledge Library: $\mathrm{CKLib}$
\STATE \quad Oracle cost: $\mathrm{OracleCost}$
\STATE \quad Exploration budget: $\mathrm{Budget}$ (used if no user goal)

\STATE \textbf{Initialize} conversation memory $\mathcal{M}$ with $(\mathcal{U}, \mathcal{E}, \text{multimodal data})$
\STATE \textbf{Initialize} incomplete causal graph $G \leftarrow \mathrm{CKLib.createGraph}(\mathcal{U}, \mathcal{E})$

\FOR{step = 1 to \text{maxSteps}}
    \STATE Construct an LLM prompt with:
    \STATE \quad $\bullet$ \text{User query + environment info}
    \STATE \quad $\bullet$ \text{Current memory $\mathcal{M}$ (Observations, prior steps)}
    \STATE \quad $\bullet$ \text{Instructions for ReAct output format (Thought, Action, Action Input, Answer)}

    \STATE \textbf{LLM} $\rightarrow$ \{\textit{Thought}, \textit{Action}, \textit{Action Input}, \textit{Answer}\}
    
    \IF{\textit{Answer} is not empty}
        \RETURN \textit{Answer} \quad \COMMENT{Stop and return final answer}
    \ELSIF{\textit{Action} = \texttt{CausalRefinementAndAction}}
        \STATE \textbf{Observation} $\leftarrow$ \textproc{CausalRefinementAndActionSubroutine}\bigl(\textit{Action Input}, G, \mathrm{CKLib}, \mathrm{OracleCost}, \mathrm{Budget}\bigr)
        \STATE Update conversation memory: $\mathcal{M} \leftarrow \mathcal{M} \cup \{\textbf{Observation}\}
    \ELSIF{\textit{Action} = \texttt{AnyOtherTool}}
        \STATE \textbf{Observation} $\leftarrow$ \textproc{CallTool}(\textit{Action Input})
        \STATE Update conversation memory: $\mathcal{M} \leftarrow \mathcal{M} \cup \{\textbf{Observation}\}
    \ELSE
        \STATE \textbf{Observation} $\leftarrow$ \texttt{UnknownAction}
        \STATE Update conversation memory: $\mathcal{M} \leftarrow \mathcal{M} \cup \{\textbf{Observation}\}
    \ENDIF
\ENDFOR

\end{algorithmic}
\end{algorithm}


\begin{algorithm}[H]
\caption{\texttt{CausalRefinementAndActionSubroutine}}
\label{alg:causal-refine-act}
\begin{algorithmic}[1]
\REQUIRE $G$: current causal graph
\REQUIRE \textit{Action Input}: instructions from the LLM (e.g., refine or plan steps)
\REQUIRE $\mathrm{CKLib}$: causal knowledge library
\REQUIRE $\mathrm{OracleCost}$, $\mathrm{Budget}$

\STATE \textbf{Parse} \textit{Action Input} to see:
\STATE \quad (i) if a refinement is requested,
\STATE \quad (ii) if a plan execution step is requested,
\STATE \quad (iii) if both refinement and partial plan execution are required.

\STATE \textbf{Refinement (if requested or if $G$ is incomplete):}
\STATE \quad $(\Delta G, \mathrm{Gain}) \leftarrow \mathrm{CKLib.estimateRefinement}(G)$
\IF{$\mathrm{Gain}$ is significant}
  \STATE $(\mathrm{InterventionCost}, \mathrm{InterventionAction}) \leftarrow \mathrm{CKLib.estimateInterventionCost}(\Delta G)$
  \IF{$\mathrm{InterventionCost} < \mathrm{OracleCost}$}
    \STATE Perform $\mathrm{InterventionAction}$ in the environment
    \STATE $\mathrm{Obs} \leftarrow \text{read environment outcomes}$
    \STATE $G \leftarrow \mathrm{CKLib.update}(G, \mathrm{Obs})$
  \ELSE
    \STATE $\mathrm{OracleQuery} \leftarrow \mathrm{CKLib.formulateQuery}(\Delta G)$
    \STATE $\mathrm{OracleAnswer} \leftarrow \text{ask Oracle with }\mathrm{OracleQuery}$
    \STATE $G \leftarrow \mathrm{CKLib.update}(G, \mathrm{OracleAnswer})$
  \ENDIF
\ENDIF

\STATE \textbf{Plan and Execute (if requested):}
\STATE $\mathrm{Plan} \leftarrow \mathrm{CKLib.plan}(G)$ 
\STATE Perform zero or more steps from $\mathrm{Plan}$ in the environment (if feasible)
\STATE Gather any partial results $\mathrm{Obs}$
\STATE $G \leftarrow \mathrm{CKLib.update}(G, \mathrm{Obs})$

\STATE \textbf{Final Return:} 
\STATE \quad Summarize changes in $G$, partial plan results, or other new knowledge in an \textbf{Observation} string.

\RETURN \textbf{Observation}

\end{algorithmic}
\end{algorithm}

==> tables.tex <==
\begin{table}[h!]
\centering
\caption{Processes and Theories Underlying Causal Reasoning and Question-Making}
\begin{tabular}{|p{3cm}|p{5cm}|p{5cm}|}
\hline
\textbf{Process} & \textbf{Description} & \textbf{Relevant Theory/Study} \\ \hline
Exploration (Random and Directed) & Balancing random sampling with uncertainty-directed exploration to gain new knowledge & Exploration-Exploitation Dilemma \cite{meder2021development} \\ \hline
Question Formulation & Identifying knowledge gaps and framing questions to obtain specific information & Developmental Question-Asking Framework \cite{ronfard2018question} \\ \hline
Causal Inference & Drawing conclusions about relationships between causes and effects & Causal Reasoning and Scientific Literacy \cite{booth2022causal} \\ \hline
Counterfactual Reasoning & Evaluating hypothetical scenarios to understand alternative causal paths & Counterfactual Reasoning and Experimentation \cite{walker2020asking} \\ \hline
Generalization & Using inductive reasoning to predict and explore novel options & Inductive Generalization in Childhood \cite{meder2021development} \\ \hline
\end{tabular}
\label{table:processes_theories}
\end{table}


\begin{table}[h!]

\centering

\caption{Tasks for Evaluating Processes Underlying Causal Reasoning and Question-Making}

\begin{tabular}{|p{3cm}|p{3cm}|p{5cm}|p{3cm}|}

\hline

\textbf{Task Name} & \textbf{Process} & \textbf{Description} & \textbf{Reference} \\ \hline

Explore-Exploit Game & Exploration (Random and Directed) & Simulates decision-making under uncertainty where agents choose between exploring unknown options or exploiting known rewards & \cite{meder2021development} \\ \hline

"Why and What If?" Scenario Task & Question Formulation and Counterfactual Reasoning & Prompts agents to generate "why" and "what if" questions to explain causal mechanisms and evaluate hypothetical outcomes & \cite{walker2020asking} \\ \hline

Causal Chain Discovery & Causal Inference & Requires agents to identify and verify causal relationships in sequential interactions or events & \cite{booth2022causal} \\ \hline

Hypothesis Testing Maze & Generalization & Agents navigate a maze, making predictions about paths based on prior experience and inductive reasoning & \cite{meder2021development} \\ \hline

Epistemic Question Challenge & Question Formulation & Assesses the agent’s ability to identify knowledge gaps and frame precise questions to obtain specific information & \cite{ronfard2018question} \\ \hline

\end{tabular}

\label{table:tasks_processes}

\end{table}
